Security, Privacy, and Decentralization in Web3

Much of the recent excitement around decentralized finance (DeFi) comes from hopes that DeFi can be a secure, private, less centralized alternative to traditional finance systems. However, people moving to DeFi sites in hopes of improving their security and privacy may end up with less of both as recent attacks have demonstrated. In this work, we improve the understanding of DeFi by conducting the first Web measurements of the security, privacy, and decentralization properties of popular DeFi front ends. We find that DeFi applications -- or dapps -- suffer from the same security and privacy risks that frequent other parts of the Web but those risks are greatly exacerbated considering the money that is involved in DeFi. Our results show that a common tracker can observe user behavior on over 56% of websites we analyzed and many trackers on DeFi sites can trivially link a user's Ethereum address with PII (e.g., user name or demographic information), or phish users by initiating fake Ethereum transactions. Lastly, we establish that despite claims to the opposite, because of companies like Amazon and Cloudflare operating significant Web infrastructure, DeFi as a whole is considerably less decentralized than previously believed.

==> sections/08_acknowledgements.tex <==
\section*{Acknowledgements}

We thank Will Scott, Roman Semenov, Arthur Gervais, Jens Ernstberger, Hamed Haddadi, and Gonçalo Pestana for their feedback on our work.
